An obstacle to a decomposition theorem for near-regular matroids

Seymour's Decomposition Theorem for regular matroids states that any matroid representable over both GF(2) and GF(3) can be obtained from matroids that are graphic, cographic, or isomorphic to R10 by 1-, 2-, and 3-sums. It is hoped that similar characterizations hold for other classes of matroids, notably for the class of near-regular matroids. Suppose that all near-regular matroids can be obtained from matroids that belong to a few basic classes through k-sums. Also suppose that these basic classes are such that, whenever a class contains all graphic matroids, it does not contain all cographic matroids. We show that in that case 3-sums will not suffice.

==> defs.tex <==
\usepackage{amsmath,amsthm,amscd}% AMS macros and such


% General font options
%\usepackage[T1]{fontenc}
%\usepackage{textcomp}

\def\SvZrequireslantedRedef{0}
\ifcase\SvZfontcode
% 0 - Computer Modern
% Default; no package needed.
\usepackage{bm}% bold symbols
\usepackage{amssymb}
\def\SvZrequireslantedRedef{1}
\or
% 1 - Fourier + New Century Schoolbook  **** (maar heeft nogal een "boek" uitstraling)
\usepackage{fouriernc}
\usepackage{bm}% bold symbols
\def\SvZrequireslantedRedef{1}
\or
% 2 - Fourier + Utopia  ****
\usepackage{fourier}
\usepackage{bm}% bold symbols
\def\SvZrequireslantedRedef{1}
\or
% 3 - Times ***
\usepackage{amssymb}
\if\SvZslantedGreekCapitals 1
\usepackage[slantedGreek]{mathptmx}
\else
\usepackage{mathptmx}
\fi
\DeclareMathAlphabet{\bm}{OT1}{ptm}{b}{it} % Apparently this creates boldface. It is better than bm, but doesn't make symbols bold.
\or
% 4 - Kerkis *
\usepackage{kmath,kerkis}
\usepackage{bm}% bold symbols
\def\SvZrequireslantedRedef{1}
\or
% 5 - Palatino    (too wide to my liking) *
\if\SvZslantedGreekCapitals 1
\usepackage[sc,slantedGreek]{mathpazo}
\else
\usepackage[sc]{mathpazo}
\fi
\usepackage{bm}% bold symbols
\linespread{1.05}
\or
% 6 - Mathdesign + Utopia
\usepackage[adobe-utopia]{mathdesign}
\usepackage{bm}% bold symbols
\or
% 7 - Garamond
\usepackage[urw-garamond]{mathdesign}
\usepackage{bm}% bold symbols
\or
% 8 - Charter
\usepackage[bitstream-charter]{mathdesign}
\usepackage{bm}% bold symbols
\or
% 9 - Latin Modern
\usepackage{lmodern}
\usepackage{bm}% bold symbols
\def\SvZrequireslantedRedef{1}
\or
% 10 - Arev: sans serif for presentations
\usepackage{arev}
% Experiments with other fonts:
%\usepackage{cmbright}
%\usepackage[math]{iwona}
%\usepackage[math]{kurier}
\fi

\if\SvZrequireslantedRedef 1
\if\SvZslantedGreekCapitals 1
% The straight capitals are saved in new variables first
\let\straightGamma\Gamma
\let\straightDelta\Delta
\let\straightTheta\Theta
\let\straightLambda\Lambda
\let\straightXi\Xi
\let\straightPi\Pi
\let\straightSigma\Sigma
\let\straightUpsilon\Upsilon
\let\straightPhi\Phi
\let\straightPsi\Psi
\let\straightOmega\Omega
\renewcommand{\Gamma}{\varGamma}
\renewcommand{\Delta}{\varDelta}
\renewcommand{\Theta}{\varTheta}
\renewcommand{\Lambda}{\varLambda}
\renewcommand{\Xi}{\varXi}
\renewcommand{\Pi}{\varPi}
\renewcommand{\Sigma}{\varSigma}
\renewcommand{\Upsilon}{\varUpsilon}
\renewcommand{\Phi}{\varPhi}
\renewcommand{\Psi}{\varPsi}
\renewcommand{\Omega}{\varOmega}
\fi
\fi
% I also have a preference for varphi over phi
\let\straightphi\phi
\renewcommand{\phi}{\varphi}
% === End of font section ===

% Change the side of the marginpar
\reversemarginpar



% Safe to use packages, even if we are in a presentation
\usepackage{url}
\usepackage{listings}
\lstset{language=C++,tabsize=4,breaklines=true}
\usepackage{kbordermatrix}
\usepackage{booktabs}
\usepackage{graphicx}
\usepackage{color}

\ifx\SvZinPresentation\undefined
% We are NOT in a presentation. Then it is safe to use also the following packages.
\usepackage{float}
\usepackage{longtable}
\usepackage[margin=10pt,labelfont=bf,textfont=it]{caption}

\usepackage[colorlinks]{hyperref}
% Backref provides links from the bibliography back to the places where the item was cited.
% The following lines format these references. The first eliminates multiple cites per section
% (though sometimes it could be useful to have them all there).
% \newcommand{\backrefxxxdupe}[3]{#2}
% % This does the formatting, again without duplications. Replace #1 by #3 and #2 by #4 to have all back
% % references.
% \renewcommand{\backref}[1]{}
% \renewcommand{\backrefalt}[4]{
% \ifcase #1
% % 0 - no citations
% \or
% % one citation
% Cited in Section #2.
% \else
% % more than one citation
% Cited in Sections #2.
% \fi
% }
% \fi

% Enumeration style: (i),(ii), etc.
\renewcommand{\theenumi}{\textit{\roman{enumi}}}
\renewcommand{\labelenumi}{(\theenumi)}

\newcommand{\mathds}{\mathbb}

% Cones, hulls and other stuff we sometimes need.
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\epi}{Epi}
\DeclareMathOperator{\conv}{conv.hull}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\ex}{Ex}
\DeclareMathOperator{\lin}{lin.hull}
\DeclareMathOperator{\aff}{aff.hull}
\DeclareMathOperator{\lins}{lin}
\DeclareMathOperator{\dirs}{dir}
\DeclareMathOperator{\row}{rowspace}
\DeclareMathOperator{\inth}{int}
\DeclareMathOperator{\kernel}{kernel}
\DeclareMathOperator{\rank}{rk}
\DeclareMathOperator{\inert}{inertia}
\DeclareMathOperator{\sig}{signature}
\DeclareMathOperator{\head}{head}
\DeclareMathOperator{\tail}{tail}
\DeclareMathOperator{\vol}{Volume}
\DeclareMathOperator{\pos}{P}
\DeclareMathOperator{\sos}{\Sigma}
\DeclareMathOperator{\charpol}{char.poly}

% Groups, rings and (partial) fields
\newcommand{\Q}{ \mathds{Q} }
\newcommand{\R}{ \mathds{R} }
\newcommand{\Rp}{ \mathds{R_+} }
\newcommand{\Z}{ \mathds{Z} }
\newcommand{\C}{ \mathds{C} }
\newcommand{\N}{\mathds{N}}
\newcommand{\field}{\mathds{F}}
\newcommand{\group}{G}
\newcommand{\bracketring}{\mathds{B}}
\DeclareMathOperator{\GF}{GF}
\newcommand{\ring}{R}
\newcommand{\parf}{\ensuremath{\mathbb{P}}} % partial field
\newcommand{\pf}{\parf}% I prefer this, but it clashes with Elsevier's class file
% Some specific partial fields:
\newcommand{\reg}{\uniform_0}
\newcommand{\dyadic}{\mathds{D}}
\newcommand{\nreg}{\uniform_1}
\newcommand{\psru}{\mathds{S}}
\newcommand{\sru}{\ensuremath{\sqrt[6]{1}}}
\newcommand{\golmean}{\mathds{G}}%ensuremath{\pf_{\mathrm{gm}}}}
\newcommand{\golrat}{\mathds{G}}%ensuremath{\pf_{\mathrm{gm}}}}
\newcommand{\splittable}{\mathds{Y}}
\newcommand{\ger}{\mathds{GE}}
\newcommand{\gauss}{\hydra_2}
\newcommand{\hydra}{\mathds{H}}
\newcommand{\cyclo}{\mathds{K}}
\newcommand{\kreg}{\mathds{U}}
\newcommand{\uniform}{\mathds{U}}
\newcommand{\fund}{\ensuremath{{\cal F}}}
\DeclareMathOperator{\cra}{cr}% cross ratio
\DeclareMathOperator{\crat}{Cr}% cross ratios
\newcommand{\Crat}{\crat}
\DeclareMathOperator{\assoc}{Asc}% associates (symmetry group of fund. elt. under 1-p and 1/p)
\DeclareMathOperator{\fun}{{\cal F}}
\newcommand{\lift}{\mathds{L}}
\newcommand{\dowling}{\mathds{D}}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\hat}{\widehat}
\renewcommand{\bar}{\overline}

% Commands to work with drafts
\newcommand{\ignore}[1]{}
\newcommand{\todo}[1]{\textsl{\small[#1]}\marginpar{\tiny\textsc{To Do!}}}

% Sixth-root-of-unity
\newcommand{\even}{\mathrm{even}}
\newcommand{\odd}{\mathrm{odd}}
\newcommand{\positive}{+}
\newcommand{\negative}{-}
\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\lc}{\sqcap}
\DeclareMathOperator{\closure}{cl}

% Some matroids
\DeclareMathOperator{\matroid}{M}
\DeclareMathOperator{\PG}{PG} % projective geometry
\DeclareMathOperator{\AG}{AG} % projective geometry
\newcommand{\deltadot}{Q^+}%{\mathaccent\cdot\triangle}

% Some structures leading to matroids
\newcommand{\wheel}[1]{\mathcal{W}_{#1}}
\newcommand{\whirl}[1]{\mathcal{W}^{#1}}

\newcommand{\oddKfour}{\ensuremath{-K_4}}
\newcommand{\Cthreetwo}{\ensuremath{\pm K_3}}
\newcommand{\Tsix}{\ensuremath{T_6}}

% SetMinus
% Redefined to differ between this and minors.
\let\Oldsetminus\setminus
%\renewcommand{\setminus}{\ensuremath{-}}

% Minors
\newcommand{\delete}{\ensuremath{\!\Oldsetminus\!}}
\newcommand{\contract}{\ensuremath{\!/}}
\newcommand{\symdiff}{\triangle}
\newcommand{\minorof}{\ensuremath{\preceq}}

\newcommand{\dirE}{\overrightarrow{E}}
\newcommand{\dirG}{\overrightarrow{G}}

% The B-fundamental circuit incidence matrix of M:
\newcommand{\fuma}{D^\#}
% The bipartite graph associated with a matrix: rows and columns are vertices; nonzero entries are edges.
\newcommand{\bip}{G}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}{Claim}[theorem] % For partial results within a proof
\newtheorem{aclaim}{Claim}[theorem] % For partial results within a proof - this solves a clash with Elsevier's class file
\newtheorem{sclaim}{Claim}[claim] % For partial results within a claim
\newtheorem{iclaim}[theorem]{Claim} % For ``independent'' claims, such as halfway an algorithm
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{falsity}[theorem]{Falsity}

% Provide an environment for indenting claims
\newenvironment{claimenv}{\list{}{\rightmargin0pt\leftmargin10pt\topsep0pt}\item[]}{\endlist}

% subproof environment
\newenvironment{subproof}{\begin{claimenv}\begin{proof}}{\end{proof}\end{claimenv}}
% These are not in the Beamer package
\newtheorem{question}[theorem]{Question}
\newtheorem{quest}[theorem]{Quest} 
